SynBullying: A Multi LLM Synthetic Conversational Dataset for Cyberbullying Detection

We introduce SynBullying, a synthetic multi-LLM conversational dataset for studying and detecting cyberbullying (CB). SynBullying provides a scalable and ethically safe alternative to human data collection by leveraging large language models (LLMs) to simulate realistic bullying interactions. The dataset offers (i) conversational structure, capturing multi-turn exchanges rather than isolated posts; (ii) context-aware annotations, where harmfulness is assessed within the conversational flow considering context, intent, and discourse dynamics; and (iii) fine-grained labeling, covering various CB categories for detailed linguistic and behavioral analysis. We evaluate SynBullying across five dimensions, including conversational structure, lexical patterns, sentiment/toxicity, role dynamics, harm intensity, and CB-type distribution. We further examine its utility by testing its performance as standalone training data and as an augmentation source for CB classification.

==> 0-abstract.tex <==
%
% moveing abstract back to main tex file as latex complain about maketitleabstract command part of the lrec template if we use \input{}
%


%Results show that LLaMA most closely reproduces authentic lexical and toxicity patterns, Grok produces highly adversarial content, and GPT-4o yields overly sanitized yet diverse dialogues. Classifier experiments demonstrate that synthetic data cannot replace human-authored samples but significantly enhance robustness and cross-domain generalization when used for data augmentation. SynBullying thus provides a reproducible, ethically responsible resource for advancing context-aware CB detection and analysis.

 

==> prompt-for-labelling-old.tex <==
Note that in this prompt, we use GPT to annotate each message with a binary
\texttt{"is\_harmful"} label, \texttt{CB\_types}, and \texttt{tone\_types},
and to assign a conversation-level \texttt{"final\_status"} label.
However, in this paper, we use only the \texttt{is\_harmful} and \texttt{CB\_types}
annotations and retain the \texttt{tone\_types} and \texttt{final\_status}
labels for future analysis.

% JW: It's unlikely the following 4 lines are not part of the prompt. They look
% like Python code.
%# === PROMPT
%ANNOTATION_PROMPT = """
%...
%"""
\begin{verbatim}
Role Instruction \&
You are an expert annotator of CB (cyberbullying) conversations. I will provide you a conversation. Each turn contains: \\
- "speaker": the role of the sender (e.g., VCTM, BULLY1, VSUP1, etc.) \\
- "text": the actual message content.
\\


Your task is to carefully read the conversation and annotate each message according to the following rules:
\\

Annotation Rules:
1) Read the entire conversation to understand context. \\

2) For each message, output a JSON object keyed by its message\_id (conversation number). \\
Each object must include: \\
- "is\_harmful": "yes" or "no" \\
- "CB\_types": a list of all applicable CB types \\
• Must be empty if none apply \\
• If "is\_harmful" = "yes", must contain at least one label \\
• Multi-word types must use underscores (e.g., Insult\_Body\_Shame, Insult\_Discrimination\_Sexism) \\
- "tone\_types": a list of applicable tone labels (can be empty if none)
\\


3) Tone label definitions: \\
- "sarcasm" → when the message conveys the opposite of what is literally said, often mockingly or with ridicule \\
- "humorous" → when the message contains humor, laughter markers (lol, lmao, haha, \\ % ��), or deliberate joking (even if cruel) \\
- "hate\_speech" → when the message mocks, insults, or discriminates based on protected characteristics (color, ethnicity, gender, orientation, nationality, religion, etc.)
\\


4) Some messages may contain multiple harmful parts → assign multiple CB\_types. \\

5) After all messages, add a top-level field "final\_status" with one of the following values: \\
- "positive" → if the conversation ends in support, de-escalation, or reconciliation \\
- "negative" → if it ends without support or reconciliation \\
- To determine this, consider only the last 10 messages. \\

6) Always return JSON only, with no extra explanation text.
\\

CB Types and Examples:
1) Threat\_or\_blackmail \\
   Expressions of physical or psychological threats, or blackmail. \\
   Examples: \\
   • [I’ll punch you in the face.] \\
   • [Do as I asked or I’ll post a nude photo of you.] \\

2) Insult\_General \\
   General insults not covered by other categories. \\
   Examples: \\
   • [You’re just a dickhead] \\
   • [Spy!] \\

3) Insult\_Body\_Shame \\
   Criticism based on body shape, size, or appearance. \\
   Examples: \\
   • [You’re a fatty!] \\
   • [You have the grace of an elephant] \\

4) Insult\_Discrimination\_Sexism \\
   Sexist insults or discrimination based on sex, gender, or orientation. \\
   Examples: \\
   • [You’re too dumb to understand this, you’re just a woman.] \\
   • [What are you, some kind of tranny freak] \\

5) Insult\_Discrimination\_Racism \\
   Discrimination based on race, skin color, ethnicity, nationality, or religion. \\
   Examples: \\
   • [You’re a Jewish asshole] \\
   • [Shitty n****r] \\
   • [Southerner!] \\

6) Insult\_Attacking\_Relatives \\
   Insults aimed at relatives or friends of the victim. \\
   Examples: \\
   • [Your mother is so fat she wouldn’t fit into the Grand Canyon] \\

7) Curse\_or\_Exclusion \\
   Wishing harm, exclusion, or rejection. \\
   Examples: \\
   • [We don’t want you on the team anymore] \\
   • [Outcast of society] \\
   • [Shut up!] \\

8) Defamation \\
   Revealing embarrassing/defamatory info about the victim to a public. \\
   Examples: \\
   • [I heard that his father lost his job and became an alcoholic] \\

9) Sexual\_Talk\_Harmless \\
   Consensual or neutral sexual talk. \\
   Examples: \\
   • [I’d like to kiss you] \\

10) Sexual\_Talk\_Harassment \\
    Unwanted sexual talk or harassment. \\
    Examples: \\
    • [Send me a nude photo of you!] \\

11) Encouragement\_to\_Harassment \\
    Expressions supporting harassment. \\
    Examples: \\
    • [Ahah, you’re right!] \\

12) Other \\
    Any other harmful utterances not listed above. \\
    Examples: \\
    • [You’re a shitty 04]
\\

Note:
Harmful messages written by the victim should be annotated with the corresponding type of insult.

% TODO: JW: extra vspace needed here?

Example Conversation and Output:
1. BULLY1: "You’re so stupid!" \\
2. VCTM: "I didn’t mean that, sorry." \\
3. VSUP1: "Hey, let’s calm down." \\
4. BULLY1: "Wow, you’re such a genius \\ % ��" \\
5. VSUP2: "Enough already. Let’s move on"
\\

Expected JSON Output \&    % TODO: check line
\texttt{\{} \\
\texttt{"1": \{"is\_harmful": "yes", "CB\_types": ["Insult\_General"], "tone\_types": []\},} \\
\texttt{"2": \{"is\_harmful": "no", "CB\_types": [], "tone\_types": []\},} \\
\texttt{"3": \{"is\_harmful": "no", "CB\_types": [], "tone\_types": []\},} \\
\texttt{"4": \{"is\_harmful": "yes", "CB\_types": ["Insult\_General"], "tone\_types": ["sarcasm", "humorous"]\},} \\
\texttt{"5": \{"is\_harmful": "no", "CB\_types": [], "tone\_types": []\},} \\
\texttt{"final\_status": "positive"} \\
\texttt{\}} \\
\texttt{"""}
\\
\begin{verbatim}

%\bottomrule
%\end{longtable}

